A Resourceful Reframing of Behavior Trees

Designers of autonomous agents, whether in physical or virtual environments, need to express nondeterminisim, failure, and parallelism in behaviors, as well as accounting for synchronous coordination between agents. Behavior Trees are a semi-formalism deployed widely for this purpose in the games industry, but with challenges to scalability, reasoning, and reuse of common sub-behaviors. We present an alternative formulation of behavior trees through a language design perspective, giving a formal operational semantics, type system, and corresponding implementation. We express specifications for atomic behaviors as linear logic formulas describing how they transform the environment, and our type system uses linear sequent calculus to derive a compositional type assignment to behavior tree expressions. These types expose the conditions required for behaviors to succeed and allow abstraction over parameters to behaviors, enabling the development of behavior "building blocks" amenable to compositional reasoning and reuse.

==> metatheory.tex <==
% \label{sec:metatheory}
% 
% The theorems stated below are primarily guiding principles for
% understanding what information is afforded by the type system and
% operational semantics. Their proofs are sketched.
% 
% \emph{Theorem 1.}
% BTL operational semantics repects congruence:
% If $\eval{\alpha}{\Delta}{\delta}$ and $\alpha \cong \beta$ then
% $\eval{\beta}{\Delta}{\delta}$.
% 
% Proof by cases on the definition of structural congruence. \qed
% 
% \emph{Theorem 2.}
% Type system correctness with respect to operational semantics:
% If $\alpha : N$ and $\eval{\alpha}{\Delta}{\Delta'}$ then
% $\Delta, N \logpre \Delta'$
% 
% Proof by simultaneous induction on the typing and evaluation derivations.
% All cases are straightforward except for sequences, for which the subcase
% involving using effects to satisfy dependencies is the main nontrivial one. 
% 
% That case proceeds as follows:
% 
% \todo{Show the seq(S1, S2-oN) case here}
% 

